Forgetting Transformer: Softmax Attention with a Forget Gate

An essential component of modern recurrent sequence models is the forget gate. While Transformers do not have an explicit recurrent form, we show that a forget gate can be naturally incorporated into Transformers by down-weighting the unnormalized attention scores in a data-dependent way. We name this attention mechanism Forgetting Attention and the resulting model the Forgetting Transformer (FoX). We show that FoX outperforms the Transformer on long-context language modeling, length extrapolation, and short-context downstream tasks, while performing on par with the Transformer on long-context downstream tasks. Moreover, it is compatible with the FlashAttention algorithm and does not require any positional embeddings. Several analyses, including the needle-in-the-haystack test, show that FoX also retains the Transformer's superior long-context capabilities over recurrent sequence models such as Mamba-2, HGRN2, and DeltaNet. We also introduce a "Pro" block design that incorporates some common architectural components in recurrent sequence models and find it significantly improves the performance of both FoX and the Transformer. Our code is available at https://github.com/zhixuan-lin/forgetting-transformer.

==> tables/lm_eval_long.tex <==
\begin{table}
\caption{Evaluation results on LM-eval-harness with $32$B training tokens and $760$M non-embedding-parameter models. "acc-n" means length-normalized accuracy. Bold and underlined numbers indicate the best and the second best results, respectively.}
\label{table:lm-eval-long}
\begin{center}
\resizebox{\columnwidth}{!}{

\begin{tabular}{l|cc|cccccccccc|c}
\toprule
\textbf{Model} & \textbf{Wiki.} & \textbf{LMB.} & \textbf{LMB.} & \textbf{PIQA} & \textbf{Hella.} & \textbf{Wino.} & \textbf{ARC-e} & \textbf{ARC-c} & \textbf{COPA} & \textbf{OBQA} & \textbf{SciQA} & \textbf{BoolQ} & \textbf{Avg} \\
 & ppl$\downarrow$ & ppl$\downarrow$ & acc$\uparrow$ & acc$\uparrow$ & acc-n$\uparrow$ & acc$\uparrow$ & acc$\uparrow$ & acc-n$\uparrow$ & acc$\uparrow$ & acc-n$\uparrow$ & acc$\uparrow$ & acc$\uparrow$ & $\uparrow$ \\
\midrule
FoT (LLaMA) & \textbf{29.46} & \textbf{22.40} & \textbf{37.69} & \textbf{61.92} & \textbf{33.91} & \textbf{51.22} & \textbf{47.77} & \underline{23.72} & \textbf{65.00} & \textbf{28.20} & \textbf{81.10} & \underline{49.88} & \textbf{48.04} \\
Transformer (LLaMA) & \underline{29.57} & \underline{24.21} & \underline{36.52} & \underline{61.32} & \underline{32.84} & \underline{48.38} & \underline{46.21} & \textbf{24.74} & \underline{60.00} & \underline{27.60} & \underline{79.10} & \textbf{61.56} & \underline{47.83} \\
\bottomrule

\end{tabular}
}
\end{center}
\end{table}

==> tables/long_bench_long.tex <==
\begin{table}
\caption{Evaluation results on LongBench with $32$B training tokens and $760$M non-embedding-parameter models. Bold and underlined numbers indicate the best and the second best results, respectively.}
\label{tab:long-bench-long}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
\multirow{5}{*}{Model} & \multicolumn{3}{c}{Single-Document QA} & \multicolumn{3}{c}{Multi-Document QA}& \multicolumn{3}{c}{Summarization}& \multicolumn{3}{c}{Few-shot Learning}& \multicolumn{2}{c}{Code} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-15}
 & \rotatebox[origin=c]{45}{NarrativeQA} & \rotatebox[origin=c]{45}{Qasper} & \rotatebox[origin=c]{45}{MFQA} & \rotatebox[origin=c]{45}{HotpotQA} & \rotatebox[origin=c]{45}{2WikiMQA} & \rotatebox[origin=c]{45}{Musique} & \rotatebox[origin=c]{45}{GovReport} & \rotatebox[origin=c]{45}{QMSum} & \rotatebox[origin=c]{45}{MultiNews} & \rotatebox[origin=c]{45}{TREC} & \rotatebox[origin=c]{45}{TriviaQA} & \rotatebox[origin=c]{45}{SamSum} & \rotatebox[origin=c]{45}{LCC} & \rotatebox[origin=c]{45}{RepoBench-P} \\
\midrule
FoT (LLaMA) & \textbf{10.62} & \underline{12.17} & \textbf{20.96} & \underline{6.53} & \underline{17.82} & \textbf{5.86} & \textbf{19.4} & \textbf{11.63} & \underline{8.74} & \textbf{48.0} & \textbf{25.7} & \textbf{21.58} & \underline{5.9} & \underline{10.55} \\
Transformer (LLaMA) & \underline{9.62} & \textbf{12.52} & \underline{19.65} & \textbf{9.63} & \textbf{18.53} & \underline{4.31} & \underline{15.45} & \underline{10.85} & \textbf{9.15} & \underline{43.5} & \underline{19.9} & \underline{20.66} & \textbf{11.98} & \textbf{17.43} \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}
